Coded Computing for Fault-Tolerant Parallel QR Decomposition

QR decomposition is an essential operation for solving linear equations and obtaining least-squares solutions. In high-performance computing systems, large-scale parallel QR decomposition often faces node faults. We address this issue by proposing a fault-tolerant algorithm that incorporates `coded computing' into the parallel Gram-Schmidt method, commonly used for QR decomposition. Coded computing introduces error-correcting codes into computational processes to enhance resilience against intermediate failures. While traditional coding strategies cannot preserve the orthogonality of $Q$, recent work has proven a post-orthogonalization condition that allows low-cost restoration of the degraded orthogonality. In this paper, we construct a checksum-generator matrix for multiple-node failures that satisfies the post-orthogonalization condition and prove that our code satisfies the maximum-distance separable (MDS) property with high probability. Furthermore, we consider in-node checksum storage setting where checksums are stored in original nodes. We obtain the minimal number of checksums required to be resilient to any $f$ failures under the in-node checksum storage, and also propose an in-node systematic MDS coding strategy that achieves the lower bound. Extensive experiments validate our theories and showcase the negligible overhead of our coded computing framework for fault-tolerant QR decomposition.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk --shell-escape -pdf \"$_[0]\"" );
    }
}

==> old_proof.tex <==
\begin{theorem}
\label{overhead1}
Under the out-of-node checksum storage, the coding strategy in Construction \ref{const:G_formula1} can be designed to achieve:
\small{
\begin{align}
%T_d &=T_{all-to-all} (p_r, \frac{n^2}{P} +\frac{n}{P}) + \gamma (\frac{2n^2}{P}+\frac{2n}{P})\\
&T_{enc} = T_{allreduce}(p_r+f, \frac{fn^2}{P}) +  \gamma  \frac{fn^2}{P} \\
&= 2 \alpha \log (p_r+f) + 2 \beta \frac{p_r+f-1}{p_r+f}\cdot\frac{fn^2}{P} +\gamma \frac{p_r+f-1}{p_r+f} \cdot \frac{f n^2}{P} \\
&T_{recov} = T_{allreduce}(p_r, \frac{f_1n^2}{P}) + T_{allreduce}(2f_1, \frac{f_1 n^2}{P}) +T_{allreduce}(p_r+f_2, \frac{f_2 n^2}{P}) \\
&+ \gamma  [\frac{(2f_1+f_2)n^2}{P}  + \frac{2}{3} f_1^3] \\%= O(T_{enc}) \text{ (given that $f=o(\frac{n}{\sqrt{P}})$)}\\
&T_{post} = T_{allreduce} (p_r, \frac{2fn(n+p_c)}{P}) + f T_{broadcast}(p_r-f+1, \frac{n(n+p_c)}{P}) + \gamma  \frac{(4f+1)n(n+p_c)}{P}
\end{align}
}
\end{theorem}
\begin{proof}[Proof of Theorem  \ref{overhead1}]
\label{proof_of_overhead1}

We now prove the formulation of $T_{enc}, T_{recov}$ and $T_{post}$ for the out-of-node checksum storage. 

%in Construction \ref{const:G_formula1} (Section \ref{Gformula1_proof}), and later show how the reasonings can be adapted similarly to in-node checksum storage in Construction \ref{Gformula2} (Section \ref{Gformula2_proof}).\\

%\subsubsection{out-of-node checksum storage}
%\label{Gformula1_overhead}
%\text{ } 

\textbf{Encoding Overhead}\\
Now we proceed to present the encoding strategy to achieve the encoding overhead $T_{enc}$, which is essentially the cost for computing the checksum $C = GA$. The encoding strategy and its overhead are summarized in Lemma \ref{encoding_strategy1}.

\begin{alg} [Encoding $Q$] \label{alg:Q_enc}
Our encoding strategy  is composed of the following steps  for any $j^{th}$ block-column in parallel:
\begin{enumerate}
	\item Every processor $\Pi(t, j)$ ($t\in[0, p_r-1]$) computes: 
	\begin{align}
\label{reorder1}
\bar{A}_{\Pi(t,j)}   = 
\begin{bmatrix}
\tilg_{0,t} \cdot A_{t, j}\\
\tilg_{1,t} \cdot A_{t, j}\\
\vdots \\
\tilg_{f-1,t} \cdot A_{t, j}
\end{bmatrix}. 
\end{align}
\item The $p_r$ systematic processors $\Pi(0, j), \Pi(1, j), ..., \Pi(p_r-1, j)$ and the  $f$ checksum processors $\Pi_C(0,j), \Pi_C(1,j), ..., \Pi_C(f-1,j) $ on the $j$-th column perform MPI\_Allreduce to compute: 
\begin{align}
\label{checksum_computation1}
    \sum_{t=0}^{p_r-1}  \bar{A}_{\Pi(t,j)} + \sum_{i=0}^{f-1} \bar{V}_{i,j} = \begin{bmatrix}
\sum_{t=0}^{p_r-1} \tilg_{0,t} \cdot A_{t, j}\\
\sum_{t=0}^{p_r-1} \tilg_{1,t} \cdot A_{t, j}\\
\vdots \\
\sum_{t=0}^{p_r-1} \tilg_{f-1,t} \cdot A_{t, j}
\end{bmatrix}, 
\end{align}
% incurring $ T_{allreduce}(p_r+f, \frac{fn^2}{P}) $ overhead.
After MPI\_Allreduce, each checksum processor $\Pi_C(i,j)$ retrieves it checksum $C_{i,j}$.
\end{enumerate}
\end{alg}

\begin{lemma}
\label{encoding_strategy1}

The overhead of the encoding strategy given in Algorithm~\ref{alg:Q_enc} is:
\begin{align*}
T_{enc} &= T_{allreduce}(p_r+f, \frac{fn^2}{P}) +  \gamma  \frac{fn^2}{P} \\
&= 2 \alpha \log (p_r+f) + 2 \beta \frac{p_r+f-1}{p_r+f}\cdot\frac{fn^2}{P} +\gamma \frac{p_r+f-1}{p_r+f} \cdot \frac{f n^2}{P} 
\end{align*}
\end{lemma}

\begin{proof}[Proof of Lemma \ref{encoding_strategy1}]
Since the encoding is performed column-wise in parallel, we only consider the cost of encoding the $j$-th. column. Computing \eqref{reorder1} in the first step is done locally, so it only incurs computation cost of $\gamma  \frac{fn^2}{P}$. The all-reduce communication in the second step is $\text{MPI\_Allreduce}(p_r+f, \frac{fn^2}{P})$ operation, hence the overhead is given by $T_{allreduce}(p_r+f, \frac{fn^2}{P})$. 

% In our system model (Section \ref{sys_model}), the input  $n \times n$ matrix $A$ is divided into $p_r \times p_c$ blocks $A_{ij}$ ($i \in [0, p_r-1]$, $j \in [0, p_c-1]$), each of which is of size $b\times b$ and owned by processor $\Pi(i,j)$. In particular, for any $j^{th}$ block-column: 

% \begin{align}
% \label{checksum_matrix_2}
% \begin{bmatrix} C_{0,j} \\ C_{1,j} \\ \vdots \\ C_{f-1, j}  \end{bmatrix} = G \begin{bmatrix} A_{0,j} \\ A_{1,j} \\ \vdots \\ A_{p_r-1, j}  \end{bmatrix}
% \end{align}
% where each $A_{ij}$ is owned by processor $\Pi(i,j)$ and, under our restriction $p_r | N$ (to avoid unecessary complication), $C_{i,j}$ is owned by the checksum processor $\Pi_C(i,j)$ . 
% % It is notable that $\Pi(i,j) = \Pi(i  \mod p_r,j)$. 
% From \eqref{generator_mat1}, we can obtain the checksum $C_{i,j}$ by:
% \begin{align}
% \label{checksum_overhead1}
%     C_{i,j} = \sum_{t=0}^{p_r-1} \tilg_{i,t} A_{t, j}
% \end{align}
% We now present the strategy to compute (\ref{checksum_overhead1}). 

% \begin{observation}
% \label{fix_j1}
% The sub-index $j$ in (\ref{checksum_overhead1}) is fixed, so we only need vertical communication of data. We can design the communication of data among all the $p_r$ vertical processors $\Pi(0, j), \Pi(1, j), ..., \Pi(p_r-1, j)$ and the $f$ vertical checksum processors $\Pi_C(0,j), \Pi_C(1,j), ..., \Pi_C(p_r-1,j)$, all of which occupy data blocks on the same block-column. Each column-wise communication can run in parallel for all $j$. 
% \end{observation}


% On each processor $\Pi(t, j)$, We further compute the following $\frac{fn}{p_r} \times \frac{n}{p_c}$ matrix $\bar{A}_{\Pi(t,j)}$ to prepare data for checksum computation \eqref{checksum_overhead1}: 



% On each checksum processor $\Pi_C(i,j)$, we form the  $\frac{fn}{p_r} \times \frac{n}{p_c}$ zero matrix $\bar{V}_{i,j}$ to prepare data for checksum computation \eqref{checksum_overhead1}: 
% \begin{align}
%     \bar{V}_{i,j}  = \begin{bmatrix}
% \vect{0}_{\frac{n}{p_r} \times \frac{n}{p_c}}\\
% \vect{0}_{\frac{n}{p_r} \times \frac{n}{p_c}}\\
% \vdots \\
% \vect{0}_{\frac{n}{p_r} \times \frac{n}{p_c}}
% \end{bmatrix} 
% \end{align}

% \begin{observation}
% \label{minor_overhead1}
% The trasformation (\ref{reorder1}) incurs $\gamma  \frac{fn^2}{P}$ overhead. 
% \end{observation}
% \begin{proof}[Proof of Observation \ref{minor_overhead1}]
% Each multiplication of $\tilg_{i,t}$ ($i\in[0, f-1]$) with the matrix $A_{t, j}$ of size $\frac{n}{p_r} \times \frac{n}{p_c}$ incurs $\gamma \frac{n^2}{P}$ overhead. Since we perform $f$ such multiplications, the total overhead is $\gamma  \frac{fn^2}{P}$.
% \end{proof}
% Now to compute all the checksums on the block-column $j^{th}$ in \eqref{checksum_matrix_2}, we perform MPI\_Allreduce on the $p_r$ vertical processors $\Pi(t, j)$ ($t \in [0, p_r-1]$) with data $\bar{A}_{\Pi(t,j)} $ and $f$  vertical checksum processors $\Pi_C(i,j)$ ($i\in[0, f-1]$) with data $\bar{V}_{i,j} $ to compute the sum:
% \begin{align}
% \label{checksum_computation1}
%     \sum_{t=0}^{p_r-1}  \bar{A}_{\Pi(t,j)} + \sum_{i=0}^{f-1} \bar{V}_{i,j} = \begin{bmatrix}
% \sum_{t=0}^{p_r-1} \tilg_{0,t} \cdot A_{t, j}\\
% \sum_{t=0}^{p_r-1} \tilg_{1,t} \cdot A_{t, j}\\
% \vdots \\
% \sum_{t=0}^{p_r-1} \tilg_{f-1,t} \cdot A_{t, j}
% \end{bmatrix}, 
% \end{align}
% which is distributed among all the $p_r + f$ participating processors. Then each checksum processor $\Pi_C(i,j)$ can retrieve its checksum as $ C_{i,j} = \sum_{t=0}^{p_r-1} \tilg_{i,t} A_{t, j}$ from \eqref{checksum_computation1}. As each of the matrices ($\bar{A}_{\Pi(t,j)}$ or $\bar{V}_{i,j}$) used in the  MPI\_Allreduce call is of size $\frac{fn}{p_r}\frac{n}{p_c}= \frac{fn^2}{P}$, this incurs the overhead $T_{reduce}(p_r+f, \frac{fn^2}{P})$. 
\end{proof}


\textbf{Overhead for Multiple-node Failure Recovery}\\
Now we present the recovery process in the presence of $f$ node failures on a vertical block-column and analyze the overhead $T_{recov}$ for recovery. 

\begin{remark}
In the actual implementation, the algorithm iteratively replaces (from left to right) columns of $A$ by columns of $Q$. In the analysis below, we still keep $A$ without introducing additional notations for simplicity. However, the recovery does include $Q$-factor protection. 
\end{remark}

% On the $j^{th}$ block-column, there are $p_r$ systematic processors $\Pi(t, j)$ ($t\in[0, p_r-1]$) holding the $\frac{n}{p_r} \times \frac{n}{p_c}$ data blocks $A_{t,j}$ and $f$ checksum processors $\Pi_C(i,j)$ ($i\in[0, f-1]$) holding the $\frac{n}{p_r} \times \frac{n}{p_c}$ checksums $C_{i,j}$ computed by \eqref{checksum_matrix_2}: 

% \begin{align*}
% \begin{bmatrix} C_{0,j} \\ C_{1,j} \\ \vdots \\ C_{f-1, j}  \end{bmatrix} &= G \begin{bmatrix} A_{0,j} \\ A_{1,j} \\ \vdots \\ A_{p_r-1, j}  \end{bmatrix} 
% \end{align*}
% where by \eqref{checksum_overhead1}:
% \begin{align*}
%     C_{i,j} &= \sum_{t=0}^{p_r-1} \tilg_{i,t} A_{t, j}
% \end{align*}
Let $f_1$ and $f_2$ be the number of failures in the systematic processors and checksum processors and let $f = f_1 + f_2$. We only consider the case when we have $f$ failures since the case of fewer than $f$ failures would require smaller overhead.
% We assume that the $f = f_1 + f_2$ node failures occur on the $j^{th}$ block-column, where $f_1$ failures strike the $p_r$ systematic processors, and $f_2$ failures strike the $f$ checksum processors. 

We partition the index set  $\{0, 1, ..., p_r-1\}= \mathcal{A}_\text{fail} \cup \mathcal{A}_\text{succ}$ , where $\mathcal{A}_\text{fail}$ denotes the indices of failed nodes among the systematic nodes of the $j$-th column, i.e., 
$$\mathcal{A}_\text{fail} = \{ t |  \Pi(t, j) \text{ is a failed systematic processor} \}$$
and $\mathcal{A}_\text{succ}$ denotes the indices of successful nodes among the systematic nodes of the $j$-th column. Similarly, we partition  $\{0, 1, ..., f-1\}= \mathcal{C}_\text{fail} \cup \mathcal{C}_\text{succ}$ to denote the failed and successful node indices within the checksum nodes on the $j$-th column. Note that $|\mathcal{A}_\text{fail}| = f_1$ and  $|\mathcal{C}_\text{fail} | = f_2$. 
% Clearly, $|\mathcal{A}_\text{fail} | = f_1$ and $|\mathcal{A}_{succ} | = p_r- f_1$. Similarly, we partition $\{0, 1, ..., f-1\}= \mathcal{C}_\text{fail} \cup \mathcal{C}_\text{succ}$, where $\mathcal{C}_\text{fail} = \{ t |  \Pi_C(t, j) \text{ is a failed checksum processor} \}$ and $\mathcal{C}_\text{succ} = \{ t | \Pi_C(t, j) \text{ is an alive checksum processor} \}$. Clearly, $|\mathcal{C}_\text{fail} | = f_2$ and $|\mathcal{C}_\text{succ} | = f_1$.
The checksum equation \eqref{checksum_overhead1} of a survived checksum block can be rewritten as:
% When these $f$ failures strike, we would lose the following data blocks $\{A_{t,j} | t \in \mathcal{A}_\text{fail} \}$ and checksums $\{ C_{t,j} | t \in \mathcal{C}_\text{fail}\}$. 
% From \eqref{checksum_overhead1}, we obtain that:
\begin{align}
\label{recovery_eq1}
    C_{i,j}  - \sum_{t \in \mathcal{A}_{succ} } \tilg_{i,t} A_{t, j} &= \sum_{t \in \mathcal{A}_\text{fail} } \tilg_{i,t} A_{t, j}, \forall i\in \mathcal{C}_\text{succ}
\end{align}

Note that the LHS of \eqref{recovery_eq1} can be computed from successful nodes, and the RHS is an equation of $f_1$ data blocks from the failed nodes. Since $|\mathcal{C}_\text{succ}| = f - f_2 = f_1$, we have $f_1$ equations on $f_1$ variables. Since any square submatrix of $\widetilde{G}$ is full-rank, we can solve the above set of linear equations to retrieve all the lost data blocks $\{A_{t,j} | t\in \mathcal{A}_\text{fail} \}$. 
% \begin{observation}
% \label{obs_recover1}
% The left-hand-side of \eqref{recovery_eq1} can be computed using data blocks and checksum of non-failed processors. Furthermore, \eqref{recovery_eq1} provides $|\mathcal{C}_\text{succ} |= f_1$ equations of $|\mathcal{A}_\text{fail} |= f_1$ variables $\{A_{t,j} | t\in \mathcal{A}_\text{fail}\}$ of lost data blocks.  Since any square submatrix of $\widetilde{G}$ is full-rank, we can solve the above set of linear equations to retrieve all the lost data blocks $\{A_{t,j} | t\in \mathcal{A}_\text{fail}\}$. 
% \end{observation}

% In our proposed strategy, we proceed to first recover all the failed data blocks $\{A_{t,j} | t \in \mathcal{A}_\text{fail} \}$ following Observation \ref{obs_recover1}, and consequently use them to recover the failed checksums $\{ C_{t,j} | t \in \mathcal{C}_\text{fail}\}$. The final recovery strategy and its overhead are summarized in Lemma \ref{recovery_strategy1}.

\begin{alg}[Recovering $Q$] \label{alg:Q_recover}
Our recovery strategy  is composed of the following steps  for any $j^{th}$ block-column in parallel:
\begin{enumerate}
	\item The $(p_r-f_1)$ successful systematic processors $\Pi(t, j)$ ($t\in \mathcal{A}_\text{succ}$) compute the matrix $\bar{A}^1_{\Pi(t,j)}$:
\begin{align}
\label{recovery_reorder1}
\bar{A}^1_{\Pi(t,j)}   = 
\begin{bmatrix}
\tilg_{i_1,t} \cdot A_{t, j}\\
\tilg_{i_2,t} \cdot A_{t, j}\\
\vdots \\
\tilg_{i_{f_1},t} \cdot A_{t, j}
\end{bmatrix} , \text{ where } \mathcal{C}_\text{succ} = \{ i_1, ..., i_{f_1}\}
\end{align}
	
% 	This step incurs $\gamma  \frac{f_1n^2}{P}$ overhead. 
	\item The $(p_r-f_1)$ successful systematic processors $\Pi(t, j)$ ($t\in \mathcal{A}_\text{succ}$) and $f_1$  successful checksum processors $\Pi_C(i,j)$ ($i\in \mathcal{C}_\text{succ}$) perform MPI\_Allreduce to compute: 
	\begin{align}
\label{recovery_computation1}
   \sum_{i \in \mathcal{C}_\text{succ}} \bar{V}^1_{i,j} - \sum_{t\in \mathcal{A}_\text{succ}}  \bar{A}^1_{\Pi(t,j)}  = \begin{bmatrix}
C_{i_1, j} - \sum_{t\in \mathcal{A}_\text{succ}} \cdot A_{t, j}\\
C_{i_2, j} - \sum_{t\in \mathcal{A}_\text{succ}} \cdot A_{t, j}\\
\vdots \\
C_{i_{f_1}, j} - \sum_{t\in \mathcal{A}_\text{succ}} \cdot A_{t, j}
\end{bmatrix}, 
\end{align}
% 	described in  \eqref{recovery_computation1} ,
% 	incurring $T_{allreduce}(p_r, \frac{f_1n^2}{P})$ overhead. 
	\item Each of the $|\mathcal{C}_\text{succ} | = f_1$  vertical checksum processors $\Pi_C(i,j)$ ($i\in \mathcal{C}_\text{succ}$) computes the matrix inverse $\widehat{G}$ used in \eqref{recovery_matrix2}. This step incurs $\gamma \frac{2}{3} f_1^3$.
	\item The $|\mathcal{C}_\text{succ} | = f_1$  vertical checksum processors $\Pi_C(i,j)$ ($i\in \mathcal{C}_\text{succ}$) compute in parallel the matrix $\bar{V}^2_{i,j}  $ in  (\ref{data_prepare_recov1}) , to be used in the next step. 
% 	This step incurs $\gamma  \frac{f_1 n^2}{P}$ overhead. 
	\item The $|\mathcal{A}_\text{fail} | = f_1$ vertical processors $\Pi(t, j)$ ($t\in \mathcal{A}_\text{fail}$) and $|\mathcal{C}_\text{succ} | = f_1$  vertical checksum processors $\Pi_C(i,j)$ ($i\in \mathcal{C}_\text{succ}$) perform MPI\_Allreduce described in  \eqref{recovery_computation2} , incurring $T_{allreduce}(2f_1, \frac{f_1 n^2}{P})$ overhead. At the end of this step, we would have recovered  all the failed data blocks $\{A_{t,j} | t \in \mathcal{A}_\text{fail} \}$.
	\item All the vertical processors $\Pi(t, j)$ ($t\in [0, p_r-1]$) prepare data for the computation of \eqref{failed_checksum1} in the next step. 
% 	This step incurs $\gamma  \frac{f_2  n^2}{P}$ overhead. 
	\item All the vertical processors $\Pi(t, j)$ ($t\in [0, p_r-1]$) and $|\mathcal{C}_\text{fail} | = f_2$  vertical checksum processors $\Pi_C(i,j)$ ($i\in \mathcal{C}_\text{fail}$) perform MPI\_Allreduce described to compute \eqref{failed_checksum1},
% 	incurring $T_{allreduce}(p_r+f_2, \frac{f_2 n^2}{P})$ overhead. 
	\item After MPI\_Allreduce, each  of those $|\mathcal{C}_\text{fail} | = f_2$  vertical checksum processors $\Pi_C(i,j)$ ($i\in \mathcal{C}_\text{fail}$) retrieves it checksum $C_{i,j}$. At the end of this step, we would have recovered  all the failed checksums  $\{C_{i,j} | i \in  \mathcal{C}_\text{fail} \}$.
\end{enumerate}
\end{alg}

\begin{lemma}
\label{recovery_strategy1}
The overhead of the recovery strategy given in Algorithm~\ref{alg:Q_recover} is:
\begin{align*}
T_{recov} &= T_{allreduce}(p_r, \frac{f_1n^2}{P}) + T_{allreduce}(2f_1, \frac{f_1 n^2}{P}) +T_{allreduce}(p_r+f_2, \frac{f_2 n^2}{P}) \\
&+ \gamma  [\frac{(2f_1+f_2)n^2}{P}  + \frac{2}{3} f_1^3]
\end{align*}
\end{lemma}
\begin{proof}[Proof of Lemma \ref{recovery_strategy1}] 
We hereby explain the steps in details: 

\textbf{Step 1 + Step 2:}

In order to recover all the failed data blocks $\{A_{t,j} | t \in \mathcal{A}_\text{fail} \}$ following Observation \ref{obs_recover1}, we first have to compute the LHS of \eqref{recovery_eq1}, i.e. computing $ C_{i,j}  - \sum_{t \in \mathcal{A}_\text{succ} } \tilg_{i,t} A_{t, j}$ on every alive checksum processor $\Pi_C(i,j)$ ($ i\in \mathcal{C}_\text{succ}$). These computations are done in Step 1 and Step 2. 

Step 1: On each of the $|\mathcal{A}_\text{succ} | = p_r-f_1$ vertical processors $\Pi(t, j)$ ($t\in \mathcal{A}_\text{succ}$), we further compute the following $\frac{f_1 n}{p_r} \times \frac{n}{p_c}$ matrix $\bar{A}^1_{\Pi(t,j)}$ to prepare data for  computation in Step 2: 
\begin{align*}
\bar{A}^1_{\Pi(t,j)}   = 
\begin{bmatrix}
\tilg_{i_1,t} \cdot A_{t, j}\\
\tilg_{i_2,t} \cdot A_{t, j}\\
\vdots \\
\tilg_{i_{f_1},t} \cdot A_{t, j}
\end{bmatrix} , \text{ where } \mathcal{C}_\text{succ} = \{ i_1, ..., i_{f_1}\}
\end{align*}


On each of the $|\mathcal{C}_\text{succ} | = f_1$  vertical checksum processors $\Pi_C(i,j)$ ($i\in \mathcal{C}_\text{succ}$), we form the  $\frac{f_1 n}{p_r} \times \frac{n}{p_c}$  matrix $\bar{V}^1_{i,j}$ to prepare data for  computation in Step 2: 
\begin{align}
    \bar{V}^1_{i,j}  = \begin{bmatrix}
\vect{0}_{\frac{n}{p_r} \times \frac{n}{p_c}}\\
\vect{0}_{\frac{n}{p_r} \times \frac{n}{p_c}}\\
\vdots \\
C_{i,j} \\
\vdots \\
\vect{0}_{\frac{n}{p_r} \times \frac{n}{p_c}}
\end{bmatrix} 
\end{align}

This step incurs $\gamma \frac{f_1n}{p_r} \times \frac{n}{p_c} = \gamma \frac{fn^2}{P}$ overhead, as each of the matrices $\bar{A}^1_{\Pi(t,j)}$ and $\bar{V}^1_{i,j}$ is of size $\frac{f_1 n}{p_r} \times \frac{n}{p_c}$. 

Step 2: we perform MPI\_Allreduce on the $|\mathcal{A}_\text{succ} | = p_r- f_1$  vertical processors $\Pi(t, j)$ ($t\in \mathcal{A}_\text{succ}$) with data $\bar{A}_{\Pi(t,j)} $ and $|\mathcal{C}_\text{succ} | = f_1$  vertical checksum processors $\Pi_C(i,j)$ ($i\in \mathcal{C}_\text{succ}$) with data $\bar{V}_{i,j} $ to compute the sum:
\begin{align}
\label{recovery_computation1}
   \sum_{i \in \mathcal{C}_\text{succ}} \bar{V}^1_{i,j} - \sum_{t\in \mathcal{A}_\text{succ}}  \bar{A}^1_{\Pi(t,j)}  = \begin{bmatrix}
C_{i_1, j} - \sum_{t\in \mathcal{A}_\text{succ}} \cdot A_{t, j}\\
C_{i_2, j} - \sum_{t\in \mathcal{A}_\text{succ}} \cdot A_{t, j}\\
\vdots \\
C_{i_{f_1}, j} - \sum_{t\in \mathcal{A}_\text{succ}} \cdot A_{t, j}
\end{bmatrix}, 
\end{align}
which is distributed among all the $p_r$ participating processors. Then each checksum processor $\Pi_C(i,j)$ can retrieve  $C_{i, j} - \sum_{t\in \mathcal{A}_\text{succ}} \cdot A_{t, j}$ from \eqref{recovery_computation1}. As each of the matrices ($\bar{A}^1_{\Pi(t,j)}$ or $\bar{V}^1_{i,j}$) used in the  MPI\_Allreduce call is of size $\frac{f_1 n}{p_r}\frac{n}{p_c}= \frac{f_1n^2}{P}$, this incurs the overhead $T_{allreduce}(p_r, \frac{f_1 n^2}{P})$. 


\textbf{Step 3:} 

By Observation \ref{obs_recover1}, the recovery of the failed data blocks can be done via \eqref{recovery_eq1}, which can be equivalently written in matrix form:
\begin{align}
\label{recovery_matrix1}
\widehat{C} = (\widehat{G} \otimes I_{n/p_r} ) \widehat{A}  
\end{align}
where:
\begin{align}
   \widehat{C} &= \begin{bmatrix}
C_{i_1, j} - \sum_{t\in \mathcal{A}_\text{succ}} \cdot A_{t, j}\\
C_{i_2, j} - \sum_{t\in \mathcal{A}_\text{succ}} \cdot A_{t, j}\\
\vdots \\
C_{i_{f_1}, j} - \sum_{t\in \mathcal{A}_\text{succ}} \cdot A_{t, j}
\end{bmatrix}  \text{ where } \mathcal{C}_\text{succ} = \{ i_1, ..., i_{f_1}\} , \\
\widehat{G} &= [\tilg_{i, t}]_{i \in \mathcal{C}_\text{succ}, t \in \mathcal{A}_\text{fail} } , \\
\widehat{A} &= \begin{bmatrix}A_{t_1, j}\\
A_{t_2, j} \\
\vdots\\
A_{t_{f_1}, j} 
\end{bmatrix}  \text{ where } \mathcal{A}_\text{fail} = \{ t_1, ..., t_{f_1}\} 
\end{align}

Since $\widetilde{G}$ is MDS, its square submatrix $\widehat{G}$ is invertible. From \eqref{recovery_matrix1}, the failed data blocks $\widehat{A}$ can be recovered by:
\begin{align}
\label{recovery_matrix2}
    \widehat{A} = (\widehat{G} \otimes I_{n/p_r} )^{-1}  \widehat{C} = (\widehat{G}^{-1}\otimes I_{n/p_r} ) \widehat{C} 
\end{align}

Consequently, we first need to compute $\widehat{G}^{-1}$, which is also our Step 3 and incurs  $\gamma \frac{2}{3} f_1^3$ overhead

\textbf{Step 4 + Step 5:}

Given $\widehat{G}^{-1}$ computed from Step 3, we proceed to recover all the failed data blocks $\widehat{A}$ following \eqref{recovery_matrix2} in Step 4 and 5. In particular, \eqref{recovery_matrix2}  can be written as:
\begin{align}
    A_{t,j} = \sum_{i \in \mathcal{C}_\text{succ}} (\widehat{G}^{-1})_{t, i} \cdot \widehat{C}_{i,j} \text{ , for } t \in \mathcal{A}_\text{fail}
\end{align}

Step 4: On each of the $|\mathcal{C}_\text{succ} | = f_1$  vertical checksum processors $\Pi_C(i,j)$ ($i\in \mathcal{C}_\text{succ}$), we compute the  $\frac{f_1 n}{p_r} \times \frac{n}{p_c}$  matrix $\bar{V}^2_{i,j}$ to prepare data for  computation in Step 5: 
\begin{align}
\label{data_prepare_recov1}
    \bar{V}^2_{i,j}  = \begin{bmatrix}
(\widehat{G}^{-1})_{t_1, i} \cdot C_{i,j} \\
(\widehat{G}^{-1})_{t_2, i} \cdot C_{i,j} \\
\vdots \\
(\widehat{G}^{-1})_{t_{f_1}, i} \cdot C_{i,j} 
\end{bmatrix} 
\end{align}

 On each of the $|\mathcal{A}_\text{fail} | = f_1$ vertical processors $\Pi(t, j)$ ($t\in \mathcal{A}_\text{succ}$), we further prepare the following $\frac{f_1 n}{p_r} \times \frac{n}{p_c}$ matrix $\bar{A}^2_{\Pi(t,j)}$ to prepare data for  computation in Step 5: 
 \begin{align}
    \bar{A}^2_{\Pi(t,j)} = \begin{bmatrix}
\vect{0}_{\frac{n}{p_r} \times \frac{n}{p_c}}\\
\vect{0}_{\frac{n}{p_r} \times \frac{n}{p_c}}\\
\vdots \\
\vect{0}_{\frac{n}{p_r} \times \frac{n}{p_c}}
\end{bmatrix} 
\end{align}


Step 5: we perform MPI\_Allreduce on the $|\mathcal{A}_\text{fail} | = f_1$  vertical processors $\Pi(t, j)$ ($t\in \mathcal{A}_\text{fail}$) with data $\bar{A}^2_{\Pi(t,j)} $ and $|\mathcal{C}_\text{succ} | = f_1$  vertical checksum processors $\Pi_C(i,j)$ ($i\in \mathcal{C}_\text{succ}$) with data $\bar{V}^2_{i,j} $ to compute the sum:
\begin{align}
\label{recovery_computation2}
   \sum_{t\in \mathcal{A}_\text{succ}} \bar{A}^2_{\Pi(t,j)}+ \sum_{i \in \mathcal{C}_\text{succ}} \bar{V}^2_{i,j}     = \begin{bmatrix}
 \sum_{i \in \mathcal{C}_\text{succ}} (\widehat{G}^{-1})_{t_1, i} \cdot \widehat{C}_{i,j}\\
\sum_{i \in \mathcal{C}_\text{succ}} (\widehat{G}^{-1})_{t_2, i} \cdot \widehat{C}_{i,j}\\
\vdots \\
\sum_{i \in \mathcal{C}_\text{succ}} (\widehat{G}^{-1})_{t_{f_1}, i} \cdot \widehat{C}_{i,j}
\end{bmatrix}, 
\end{align}
which is distributed among all the $2f_1$ participating processors. Then each vertical processor $\Pi(t, j)$ ($t\in \mathcal{A}_\text{fail}$) can retrieve  $C \sum_{i \in \mathcal{C}_\text{succ}} (\widehat{G}^{-1})_{t, i} \cdot \widehat{C}_{i,j}$ from \eqref{recovery_computation2}. As each of the matrices ($\bar{A}^2_{\Pi(t,j)}$ or $\bar{V}^2_{i,j}$) used in the  MPI\_Allreduce call is of size $\frac{f_1n}{p_r}\frac{n}{p_c}= \frac{f_1 n^2}{P}$, this incurs the overhead $T_{allreduce}(2 f_1, \frac{ f_1 n^2}{P})$. 

\textbf{Step 6 + Step 7:} 

After recovering all the failed data blocks, we would proceed to recover the failed checksums:
\begin{align}
\label{failed_checksum1}
    C_{i,j} &= \sum_{t=0}^{p_r-1} \tilg_{i,t} A_{t, j}, i\in \mathcal{C}_\text{fail}
\end{align}

The computation of \eqref{failed_checksum1} is similar to that of \eqref{checksum_overhead1} in Lemma \ref{encoding_strategy1}, which computes all the checksums. We thus defer readers to the computation in Lemma \ref{encoding_strategy1} for more details, and only state the total cost of these 2 steps, which is $T_{allreduce}(p_r+f_2, \frac{f_2 n^2}{P}) + \gamma \frac{f_2 n^2}{P} $ .

\textbf{Postprocessing Overhead}\\
The overhead for postprocessing is attributed to the cost for performing matrix multiplications $(G_0 Q_1)$ and $(G_0 \bm{b})$ (refer to Section \ref{subsec:general_scheme}). By the 2D-block distribution, computing $(G_0 Q_1)$ can be broken down into parallel computations of $p_c$ block-columns $G_0 Q_1[:,0], G_0 Q_1[:,1], ..., G_0 Q_1[:,p_c-1]$. 

In our computing strategy, we denote the $n \times (\frac{n}{p_c}+1)$ matrix $Z^j = \begin{bmatrix} Q_1[:, j] & \bm{b}\end{bmatrix} = \begin{bmatrix} Z_{0} \\ Z_{1} \\ \vdots \\ Z_{p_r-1} \end{bmatrix}$, where $Z_i$ is $\frac{n}{p_r} \times (\frac{n}{p_c}+1)$ . Then the postprocessing overhead is the cost for performing matrix multiplication $G_0 Z^j$ (as we compute $G_0 Z^0, G_0 Z^1, ..., G_0 Z^{p_r-1}$ in parallel), which is further expressed as the followings to utilize the sparsity of $G_0$:
\begin{align}
G_0 Z^j &= \begin{bmatrix}
I_{\frac{fn}{p_r}}+G_1 & V \\
V^T & -I_{n-\frac{fn}{p_r}}
\end{bmatrix} Z^j  \\
&= \begin{bmatrix}
H \otimes I_{\frac{n}{p_r}} & \widetilde{V} \otimes I_{\frac{n}{p_r}} \\
\widetilde{V}^T \otimes I_{\frac{n}{p_r}}  & -I_{p_r - f} \otimes I_{\frac{n}{p_r}} 
\end{bmatrix} \begin{bmatrix} Z^j_{0} \\ Z_{1} \\ \vdots \\ Z^j_{p_r-1} \end{bmatrix}  \text{ where $H = (I_f+\widetilde{G}_1)$} \\
&= \begin{bmatrix} \sum_{i=0}^{f-1} H_{0,i} \cdot Z^j_i + \sum_{t=f}^{p_r-1} \widetilde{V}_{0,t} \cdot  Z^j_t  \\ 
\sum_{i=0}^{f-1} H_{1,i} \cdot Z^j_i + \sum_{t=f}^{p_r-1} \widetilde{V}_{1,t} \cdot  Z^j_t  \\ 
\vdots \\
\sum_{i=0}^{f-1} H_{f-1,i} \cdot Z^j_i + \sum_{t=f}^{p_r-1} \widetilde{V}_{f-1,t} \cdot  Z^j_t  \\ 
\sum_{i=0}^{f-1} \widetilde{V}_{i,0} \cdot  Z^j_i   - Z^j_{f}\\
\sum_{i=0}^{f-1} \widetilde{V}_{i,1} \cdot  Z^j_i   - Z^j_{f+1}\\
\vdots \\
\sum_{i=0}^{f-1} \widetilde{V}_{i,p_r-f-1} \cdot  Z^j_i   - Z^j_{p_r-1}\\
\end{bmatrix} 
=\begin{bmatrix} W_0 \\W_1 \\ \vdots \\ W_{p_r-1} \end{bmatrix} 
\end{align}

%To better illustrate the intuition, we consider the case where blockszie $b = \frac{n}{p_r} (=c)$. The overhead for the generalized case is the same as the case $b = \frac{n}{p_r}$, and is briefly explained in a sketchy proof later. When $b = \frac{n}{p_r}=c$, each processor $\Pi(i, t)$ holds $\frac{N}{p_c} $ block-columns of $Z_i$, where all the processors $\Pi(0, t), \Pi(1, t), \Pi(2, t), ... , \Pi(p_r-1, t)$ together occupy the whole $t^{th}$ block-column of $Z$.

Our goal is to compute $G_0 Z^j =\begin{bmatrix} W_0 & W_1 & \cdots & W_{p_r-1} \end{bmatrix}^T $ 2D-block-distributed  over the $p_r$ vertical systematic processors $\Pi(0, j), \Pi(1, j), ..., \Pi(p_r-1, j)$. 

The final postprocessing strategy and its overhead are summarized in Lemma \ref{decoding_strategy1}.

\begin{lemma}
\label{decoding_strategy1}

Our postprocessing strategy  is composed of the following steps computed in parallel on all the block-columns:
\begin{enumerate}
\item All the vertical processors $\Pi(t, j)$ ($t\in [0, p_r-1]$) compute in parallel the matrix $\bar{D}^1_{\Pi(t,j)}  $ in  \eqref{D1.1} (for $t < f$) and \eqref{D1.2} (for $t \geq f$). This step prepares data for computing $\sum_{i=0}^{f-1} H_{k,i} \cdot Z^j_i$ ($k\in [0, f-1]$) in Step 3, and incurs $\gamma  \frac{fn(n+p_c)}{P}$ overhead. 
%\item All the vertical processors $\Pi(t, j)$ ($t\in [0, p_r-1]$) compute in parallel the matrix $\bar{D}^2_{\Pi(t,j)}  $ in  \eqref{D2.1} (for $t < f$) and \eqref{D2.2} (for $t \geq f$). This step prepares data for computing $\sum_{i=0}^{f-1} \widetilde{V}_{i,k} \cdot  Z^j_i$ ($k\in [0, p_r-f-1]$) in Step 4, and incurs $\gamma  \frac{(p_r-f)n(n+1)}{P}$ overhead. 
\item All the vertical processors $\Pi(t, j)$ ($t\in [0, p_r-1]$) compute in parallel the matrix $\bar{D}^3_{\Pi(t,j)}  $ in  \eqref{D3.1} (for $t < f$) and \eqref{D3.2} (for $t \geq f$). This step prepares data for computing $\sum_{t=f}^{p_r-1} \widetilde{V}_{k,t} \cdot  Z^j_t $ ($k\in [0, f-1]$) in Step 3, and incurs $\gamma  \frac{fn(n+p_c)}{P}$ overhead. 
\item Compute $\sum_{i=0}^{f-1} H_{k,i} \cdot Z^j_i$ ($k\in [0, f-1]$),  and $\sum_{t=f}^{p_r-1} \widetilde{V}_{k,t} \cdot  Z^j_t $ ($k\in [0, f-1]$) through one  MPI\_Allreduce call incurring $T_{allreduce} (p_r, \frac{2fn(n+p_c)}{P})$ overhead.
\item Each of the first $f$ vertical processors $\Pi(t, j)$ ($t\in [0, f-1]$) sequentially broadcasts its data $Z^j_t$ to  other $(p_r-f)$ vertical processors $\Pi(k, j)$ ($k \in [f, p_r]$), incurring $f \cdot T_{broadcast}(p_r-f+1, \frac{n(n+p_c)}{P}) $ overhead. (Note: The cost can be further reduced if we use multi-broadcast).
\item Each of the  $p_r-f$ vertical processors $\Pi(k, j)$ ($k \in [f, p_r]$) computes in parallel the sum $ \sum_{i=0}^{f-1} \widetilde{V}_{i,k-f} \cdot  Z^j_i$, incurring $\gamma  \frac{2fn(n+p_c)}{P}$ overhead. 
\item Compute all $W_i$'s in parallel, incurring $\gamma \frac{n(n+p_c)}{P}$ overhead.
\end{enumerate}
The overhead of this  strategy is : 
\begin{align*}
T_{post} &= T_{allreduce} (p_r, \frac{2fn(n+p_c)}{P}) + T_{broadcast}(p_r-f+1, \frac{n(n+p_c)}{P}) + \gamma  \frac{(4f+1)n(n+p_c)}{P}
\end{align*}
\end{lemma}

\begin{proof}[Proof of Lemma \ref{decoding_strategy1}] 

We further break down the  steps in details. 

\textbf{Step 1:}

On each of the vertical processors $\Pi(t, j)$ ($t\in [0, p_r-1]$), we compute in parallel the matrix $\bar{D}^1_{\Pi(t,j)} $ by:
\begin{align}
    \bar{D}^1_{\Pi(t,j)} &= \begin{bmatrix}
    H_{0,t} \cdot Z^j_t \\
    H_{1,t} \cdot Z^j_t \\
    \vdots \\
    H_{f-1,t} \cdot Z^j_t 
    \end{bmatrix} , \text{ if $t < f $}  \label{D1.1}\\ 
    \bar{D}^1_{\Pi(t,j)} &=\begin{bmatrix}
    \vect{0}_{\frac{n}{p_r} \times (\frac{n}{p_c}+1)} \\
    \vect{0}_{\frac{n}{p_r} \times (\frac{n}{p_c}+1)} \\
    \vdots \\
    \vect{0}_{\frac{n}{p_r} \times (\frac{n}{p_c}+1)} 
    \end{bmatrix} , \text{ if $t \geq f $} \label{D1.2}
\end{align}





\textbf{Step 2:}

On each of the vertical processors $\Pi(t, j)$ ($t\in [0, p_r-1]$), we compute in parallel the matrix $\bar{D}^2_{\Pi(t,j)} $ by:
\begin{align}
    \bar{D}^2_{\Pi(t,j)} &=\begin{bmatrix}
    \vect{0}_{\frac{n}{p_r} \times (\frac{n}{p_c}+1)} \\
    \vect{0}_{\frac{n}{p_r} \times (\frac{n}{p_c}+1)} \\
    \vdots \\
    \vect{0}_{\frac{n}{p_r} \times (\frac{n}{p_c}+1)} 
    \end{bmatrix} , \text{ if $t < f $} \label{D3.1} \\
    \bar{D}^2_{\Pi(t,j)} &= \begin{bmatrix}
    \widetilde{V}_{0,t} \cdot  Z^j_t\\
    \widetilde{V}_{1,t} \cdot  Z^j_t\\
    \vdots \\
    \widetilde{V}_{f-1,t} \cdot  Z^j_t
    \end{bmatrix} , \text{ if $t \geq f $}  \label{D3.2}
\end{align}


\textbf{Step 3:}

we perform MPI\_Allreduce on all the   vertical processors $\Pi(t, j)$ ($t\in [0, p_r-1]$) with data $\bar{D}^1_{\Pi(t,j)} $ and $ \bar{D}^2_{\Pi(t,j)} $ to compute the sums:
\begin{align}
    \sum_{t=0}^{p_r-1} \bar{D}^1_{\Pi(t,j)} &= \begin{bmatrix} \sum_{i=0}^{f-1} H_{0,i} \cdot Z^j_i  \\ 
\sum_{i=0}^{f-1} H_{1,i} \cdot Z^j_i \\ 
\vdots \\
\sum_{i=0}^{f-1} H_{f-1,i} \cdot Z^j_i 
\end{bmatrix} \\
    \sum_{t=0}^{p_r-1} \bar{D}^2_{\Pi(t,j)} &=\begin{bmatrix} \sum_{t=f}^{p_r-1} \widetilde{V}_{0,t} \cdot  Z^j_t  \\ 
\sum_{t=f}^{p_r-1} \widetilde{V}_{1,t} \cdot  Z^j_t  \\ 
\vdots \\
\sum_{t=f}^{p_r-1} \widetilde{V}_{f-1,t} \cdot  Z^j_t 
\end{bmatrix} 
\end{align}
which are distributed among all the participating processors. Since  the data matrices $\bar{D}^1_{\Pi(t,j)} $ and  $ \bar{D}^2_{\Pi(t,j)} $  totally have size $2 \frac{fn}{p_r} (\frac{n}{p_c} + 1)= \frac{2fn(n+p_c)}{P}$, this step incurs $T_{allreduce} (p_r, \frac{2fn(n+p_c)}{P})$ overhead.

\textbf{Step 4:}

Since each $Z^j_t$ to be broadcasted by $\Pi(t,j)$ ($t \in [0, f-1]$) is of size $\frac{n}{p_r} \times (\frac{n}{p_c}+1)$, the cost of each MPI\_Broadcast is $T_{broadcast}(p_r-f+1, \frac{n(n+p_c)}{P}) $. As we sequentially perform $f$ such MPI\_Broadcast calls, the total overhead is $f \cdot T_{broadcast}(p_r-f+1, \frac{n(n+p_c)}{P}) $

\textbf{Step 5:}

Each of the  $p_r-f$ vertical processors $\Pi(k, j)$ ($k \in [f, p_r]$) computes in parallel the sum $ \sum_{i=0}^{f-1} \widetilde{V}_{i,k-f} \cdot  Z^j_i$, incurring $\gamma  \frac{2fn(n+p_c)}{P}$ overhead (where it takes $\gamma \frac{fn(n+p_c)}{P}$ for all the multiplications $ \widetilde{V}_{i,k-f} \cdot  Z^j_i$ and $\gamma \frac{fn(n+p_c)}{P}$ for doing the summation). 

\textbf{Step 6:}

 In parallel, each  vertical processor $\Pi(k, j)$ ($k\in [0, p_r-1]$) computes  $W_k$:
 \begin{align}
     W_k = \begin{cases} (\sum_{i=0}^{f-1} H_{k,i} \cdot Z^j_i ) +( \sum_{t=f}^{p_r-1} \widetilde{V}_{k,t} \cdot  Z^j_t )\text{ , if $k < f$} \\
   (  \sum_{i=0}^{f-1} \widetilde{V}_{i,k-f} \cdot  Z^j_i )  - Z^j_{k} \text{ , if $k \geq f$} 
     \end{cases}
 \end{align}
which is the sum of two  $\frac{n}{p_r} \times \frac{n+1}{p_c}$ matrices. The overhead of this step is thus $\gamma \frac{n(n+1)}{P}$.
\end{proof} 


\end{proof}



\end{proof}

==> problem_formulation.tex <==
\subsection{Notations and Assumptions}
We use upper-case letters to denote matrices and bold lower-case letters to denote vectors. For matrix $A$, we use $a_{i,j}$ to denote the $(i,j)$-th entry of the matrix. We use $I_m$ to denote the identity matrix of dimension $m \times m$, and write $I$ when the dimension is clear from the context. \textcolor{red}{In view of the hardness of $Q$-factor protection, the full rank of the input matrix $A$ is a technical assumption that we would impose for the post-orthogonalization framework to work. To this end, the input matrix $A$ within our interest is of size $n \times n$ and full-rank. 
The vertical and horizontal checksum generator matrices $G_v$ and $G_h$ are respectively of size $c\times n$ and $n \times d$.} 
% \hj{Check if there are other things we have to specify in the notations section}

% \textcolor{blue}{explain that for the post-orthogonalization to work, we require the matrix $A$ to be full-rank.}

\subsubsection{System Model}
\label{sys_model} 
%\hj{This should be changed to block distribution. Mention block-cyclic distribution after you explain the block distribution, and say that we think it will generalize :) }

\textbf{Processor distribution:} Let $P$ be the total number of nodes. We use \emph{nodes} and \emph{processors} interchangeably. We assume that the nodes are aligned as $p_r \times p_c$ grid ($p_r p_c = P$) and we denote the $(i,j)$-th node on the grid as $\Pi(i,j) $. We consider \emph{2D block  distribution} of a matrix (Figure \ref{fig: 2dblock}) where a  non-singular matrix  $A$ of dimension $n \times n $ ($n >> P$) is split into $p_r \times p_c$ blocks and each block $A_{ij}$ ($i\in [0, p_r-1], j\in [0,p_c-1]$) is distributed to processor $\Pi(i,j) $. 
% We are interested in large-scale computations in HPC, where failures are detrimental ~\cite{Elnozahy:2008178}, and make the practical assumption that $P\leq n$. 
The $j^{th}$ block-column is the "column" of data blocks $A_{0j}, A_{1j}, ..., A_{(p_r-1)j}$. Block-rows are defined similarly.  For simplicity, we assume that $p_r = p_c$ and consequently set the dimension of each block $A_{i,j}$ to be $b = \frac{n}{p_r} = \frac{n}{p_c}$. The 2D block distribution assumption we make here is a simplification of \emph{2D block cyclic distribution}, which is a more realistic data distribution scheme used in practical HPC algorithms.
In \emph{2D block cyclic distribution} (Figure \ref{fig: proc2}),  the number of vertical blocks  (resp. number of horizontal blocks) can be any value that is a multiple of $p_r$ (resp. $p_c$), and blocks are cyclically distributed to the nodes. 
\textcolor{blue}{While we consider 2D block distribution in this paper for simplicity of technical exposition, its code design can be used for generalization to that of 2D block cyclic distribution (by duplicating the code pattern) albeit cumbersome.}
% We believe that our results will hold with minor changes for 2D block cyclic distribution. 
% In \cite{qr_isit}, we found that the main challenge of coded QR decomposition is to restore the degraded orthogonality of the decoded Q factor (detailed discussion in Section \ref{sec:q_factor_protection} ) rather than the cyclic structure of the block distribution. In this work, we thus consider \emph{2D block  distribution} for simplicity, and believe that the results will generalize to \emph{2D block cyclic distribution}.
%HPC literature considers \emph{2D block cyclic distribution} of a matrix where a  non-singular $n \times n $ matrix  $A$ is distributed block-cyclically on $P = p_r \times p_c$ processors, and each $b_1\times b_2$ block $A_{ij}$ is owned by processor $\Pi(i,j) = ( i \text{ mod } p_r)+p_r (j \text{ mod } p_c)$. The $j^{th}$ block-column is the "column" of data blocks $A_{0j}, A_{1j}, ..., A_{(N_1-1)j}$. Block-rows are defined similarly. $N_1 = \frac{n}{b_1}$ and $N_2 = \frac{n}{b_2}$ respectively denote the number of data blocks of a block-column and a block-row. This is how matrix algorithms are implemented in practice for load balancing. A simplified version is  \emph{2D block distribution} where matrix $A$ is  divided into exactly $P$ blocks with $N_1 = p_r$ and $N_2 = p_c$ so that each processor $\Pi(i,j)$ owns exactly one block $A_{ij}$. \todo{Figure  block vs block cyclic.}

\noindent
\textbf{Failure Model:} We assume that nodes are subject to failures, especially to \emph{``fail-stop errors''}, which is a realistic failure model in HPC~\cite{fail_stop1} similar to common assumptions in the coded computing literature. In this model, a failure corresponds to a node that completely stops responding, and loses all of its data, including its inputs and computation results. 
We assume that at any \emph{iteration} of the QR decomposition at most $f$ failures can occur per column or row \textcolor{blue}{and that $f \leq \frac{1}{2}\min\{p_r, p_c\}$.}
\textcolor{red}{In order to avoid further error propagation, whereby  computation either is halted by the non-responsiveness of the failed processor or proceeds with the corrupted data, the HPC community has developed Message Passing Interface (MPI) libraries~\cite{MPI_detect_fault1} that detect the identities of the failed processors and required a global consistent state of the application be available via C/R or  reconstructed via ABFT \cite{fail_stop2}. 
To this end, we assume that  upon failure the identities of the failed processors are immediately provided by some external source and aim to develop fault-tolerant mechanism that  recovers the failed processors before proceeding the computation.}
% (e.g. Message Passing Interface (MPI) library~\cite{MPI_detect_fault1}). 
Failures can happen at any time during the computation.

\noindent
\textbf{Storage Model:} For fault-tolerance, we add encoded checksums. For storing checksums, a common assumption is \emph{out-of-node checksum storage} where we introduce additional nodes to store the checksums. We call these \emph{checksum nodes} and the nodes that store the original data, \emph{systematic nodes}. We assume that checksum nodes and systematic nodes are identical in terms of their specifications, e.g., same memory and computing power. Hence, for load balancing, we assume that all the nodes including both systematic nodes and checksum nodes process the same amount of data. Another way of storing checksums is \emph{in-of-node checksum storage}, where you store the checksums within the original set of nodes instead of introducing additional nodes. This will increase the size of the computing task per node, but it has advantages when a user wants to fix the number of nodes used for the parallel algorithm. This has been considered in~\cite{innode1}. 
In Section III, we develop a $Q$-factor protection scheme under the out-of-node checksum storage setting. In Section IV, we consider the in-node checksum storage setting and improve bounds on the number of checksums.


% \subsection{Failure Model and Real-time Recovery}\label{subsec:failure}
% We focus on recovering from \emph{``fail-stop errors''}, which is a realistic failure model in HPC~\cite{fail_stop1}, and is similar to common assumptions in coded computing. In this model, a failure corresponds to either a systematic or checksum processor that completely stops responding, and loses its  part of the global data \footnote{The failure of some systematic processor would result in the loss of its systematic data blocks, while the 
% failure of some checksum processor would result in the loss of its checksums}. 
% We assume that the identity of the processor that fails is provided by some external source (e.g. Message Passing Interface (MPI) library~\cite{MPI_detect_fault1}). 
% We focus on the \textit{multiple-node failure} scenario, i.e., at any 
% \emph{iteration} of the QR decomposition at most $f$ failures can occur per column or row. Failures can strike at any point during the execution within some iteration of QR decomposition. At the end of the iteration with failures, the system detects the identities of the failed processors and triggers the recovery process. 
% %\hj{But, we can now tolerate $f$ failures, so we do not have to trigger the recovery process immediately? Maybe we can just do this process when we have $f$ failures, or after each iteration..?} 
% Computation continues once the system has recovered from its latest failures in that iteration. 
% Figure~\ref{fig: 2dblock_fail} illustrates an example of lost data-blocks. 
% One important property facilitating real-time recovery and computing continuation from the point of failures is the checksum-preservation throughout all iterations of QR decomposition. We refer readers to \cite[Section III]{qr_isit} for more detailed discussion. 




% \subsection{MGS Algorithm}


\subsection{Checksum Generator Matrices for 2D Block Distribution}


Finally, we show how the checksum generator matrices $G_v$ and $G_h$ connect to the desired MDS property in the error-correcting codes literature. In \emph{2D block distribution}, each systematic node stores exactly one data block of size $\frac{n}{p_r} \times \frac{n}{p_c}$.
Assuming that we use the same encoding coefficients at each node for the entire data block, $G_v$ and $G_h$ can be represented as: 
\begin{align}
    G_v  = \widetilde{G}_v \otimes I_{n/p_r}, \label{tildeG_eq} \;\; G_h  = \widetilde{G}_h \otimes I_{n/p_c},
\end{align}
where $\otimes$ is a Kronecker product, $\widetilde{G}_v$ and $\widetilde{G}_h$ are respectively $m_r \times p_r$  and $p_c \times m_c$ matrices, and  $m_r$ and $ m_c$ are respectively the number of checksum nodes per row and column.
%\hj{I really don't think anything below this belongs here.. Move to Section III?} 
The desirable MDS property translates into the property of the matrices $\widetilde{G}_v$ and $\widetilde{G}_h$:
\begin{theorem}[Theorem 8, p. 321 in \cite{macwilliams1977theory}]
$\widetilde{G}_v$ (resp. $\widetilde{G}_h$) has the MDS property if and only if every square submatrix of $\widetilde{G}_v$ (resp. $\widetilde{G}_h$) is full-rank.  
\end{theorem} 

% We consider the \textit{out-of-node checksum storage:} (Figure \ref{fig: 2dblock_distribution})   The vertical (resp. horizontal) checksums are distributed over the new set of checksum processors. Each checksum processor is also prone to failures and stores the same amount of data as a systematic processor to ensure load balancing and efficient parallelism. 

% In specifically Section \ref{in_node}, we also consider the \textit{in-node checksum storage} for a broader context of any HPC matrix operation deployed on this checksum storage. Under this setting,   the vertical (resp. horizontal) checksums are distributed over the same set of systematic  nodes. Whenever a systematic node fails, we would  lose not only the data blocks, but also checksums. In general scenario where there is no restriction on the code, MDS codes can always be used for \textit{out-of-node checksum storage}, but it has remained an open question on the minimal amount of checksums required for \textit{in-node checksum storage}.

%\hj{we also consider in-node checksum.. also can we introduce $m_r$ and $m_c$ here?}



%\hj{This paragarph should be changed too..?} Despite the \emph{2D block cyclic distribution} being used in practice, the main challenge of coded QR decomposition is to restore the degraded orthogonality of the decoded Q factor (detailed discussion in Section \ref{sec:q_factor_protection} ). For simplicity, we thus consider the simplified \emph{2D block distribution} throughout the whole paper, if not stated otherwise, for our design of coding strategy and overhead analysis. Furthermore, our technique  dealing with the degraded orthogonality leverages the submatrix structure of  the vertical checksum-generator matrix $G_v = \begin{bmatrix}  G_1 & V \end{bmatrix} $ where $G_1$ and $V$ have dimensions $c \times c$ and $c \times (n-c)$, respectively. 

%In appendix \todo{fill}, we further explain how the results naturally generalize to \emph{2D block cyclic distribution} without changing the performance derivation. 

%We denote $p_c$ vertical checksum processors as $V_0, V_1, ..., V_{p_c-1}$ where $V_i$ owns the $i^{th}, (i+p_c)^{th}, (i+2p_c)^{th}, ...$ block-columns (i.e. column of $b\times b$ blocks). Similarly, we denote $p_r$ horizontal checksum processors as $H_0, H_1, ..., H_{p_r-1}$ where $H_j$ owns the $j^{th}, (j+p_r)^{th}, (j+2p_r)^{th}, ...$ block-rows (i.e. row of $b\times b$ blocks).
	

\subsection{Checksum-preservation for MGS}

Checksum-preservation is the key idea of all the previous work on coded QR decomposition including Householder \cite{colchecksum, soft_error2} and Givens Rotations \cite{givens_rotations1}. For MGS, we hereby show how horizontal and vertical checksums added to the input matrix are respectively preserved as checksums for $R$-factor and $Q$-factor throughout the computation. As the QR factorization of a rank-deficient matrix (encoded $\widetilde{A}$) is not unique, this property is not trivial and depends on specific algorithmic structure.

\noindent
\textbf{MGS algorithm:} For extreme-scale QR factorization, MGS is the favored choice thanks to its low computational cost and ease of implementation. The pseudo-code of sequential MGS is given in Algorithm \ref{alg: sequential_mgs}, where at the $i^{th}$  iteration, the algorithm computes  column $\bm{q_i}$ of the $Q$-factor and  row $\bm{r_i}$ of the $R$-factor.
For parallel implementation in practice, block MGS (BMGS) \cite{criterion1} is widely used as its parallel version (PBMGS) can better utilize the Level-3 operations in HPC. We refer to parallel MGS as PBMGS.

%The pseudo-code will be used for the intuitive proof of the checksum-preserving property in Section \ref{subsec:mgs_checksum_preserving}.




%However, our coding strategy can be adapted similarly to Givens Rotation \cite{givens_rotation2} and GS \cite{GS1} with minor modifications. For state-of-the-art implementations of Householder Transformation,  $Q$ is stored in some implicit form of  either  WY representation\footnote{WY representation is  a storage-efficient form of $Q$ introduced by \cite{WY2}} \cite{scalapack, elemental, TSQR_Householder}, or a tree of intermediate factors \cite{optimal_TSQR}. Such alternative storage of $Q$ hinders the applicability of our coding strategy for protecting $Q$. 

%In addition to the basic MGS algorithm, its variants have been developed including block versions or MGS with re-orthogonalization \cite{Barlow2019BlockMG}. 


%For illustration, we hereby present the pseudo-code for BMGS in Algorithm \ref{alg: BMGS_pseudo}. If the step size $b$ (on line 2) of BMGS is set to $b=1$, it becomes the basic MGS algorithm. 

% \vspace*{-.4cm}


\begin{algorithm}
\small
% \lstset{language=Pascal} 
% \lstset{numbers=left, numberstyle=\tiny, stepnumber=1, numbersep=5pt}
\caption{Modified Gram-Schmidt}
\SetAlgoLined
\label{alg: sequential_mgs}
\KwIn{$\widetilde{A} = \begin{bmatrix} \bm{\widetilde{a}_1} & \bm{\widetilde{a}_2} & \cdots & \bm{\widetilde{a}_{n+d}} \end{bmatrix}$ is $(n+c) \times (n+d)$ matrix}
\KwOut{$Q = \begin{bmatrix}\bm{q_1} & \bm{q_2} & \dots & \bm{q_{n+d}}\end{bmatrix}$ is $(n+c) \times (n+d)$  matrix  , and $R = (r_{ij})$ is $(n+d) \times (n+d)$  matrix}
\KwResult{$\widetilde{A} = QR$, where $Q^T Q = I$}
\For{$i=1$ \KwTo $n$ }{ 
    $\bm{u_i} = \bm{\widetilde{a}_i}$\\
    
    }
\For{$i=1$ \KwTo $n+d$ }{ 
   $r_{ii} = || \bm{u_i}||_2$ \\
   $\bm{q_i} = \bm{u_i}/r_{ii} $\\
   \For{$j=i+1$ \KwTo $n+d$ }{ 
   	$r_{ij} = \bm{q_i}^T \bm{u_j}$ \\
   	$\bm{u_{j}} = \bm{u_{j}} - r_{ij}\bm{q_i}$\\
   }
}
\end{algorithm}

\noindent
\textbf{Checksum-preservation:} The $n \times n$  matrix $A$ is  encoded as  (Section \ref{sys_model:checksum_generation}):  
\begin{align}
\label{R_checksum_preserving_equation}
\widetilde{A} = \begin{bmatrix}
	 A & A G_h\\
	 G_v A & G_v A G_h
\end{bmatrix}
\end{align}
of size $(n+c) \times (n+d)$, where $G_h$ and $G_v$ are respectively checksum-generator matrices of size $n \times d$ and $c \times n$. We assume that $c$ and $d$ are small to keep the  overhead negligible. QR decomposition via MGS is further performed on the encoded matrix $\widetilde{A}$. 
The algorithm executes $T$ iterations $t=1, \ldots, T$ where at the end of each iteration the algorithm maintains the update of the $Q$-factor $Q^{(t)} $ of size $(n+c) \times (n+d)$ and the  $R$-factor $R^{(t)}$ of size $(n+d) \times (n+d)$. The initial values of the $Q$-factor and $R$-factor are $Q^{(0)}=\widetilde{A}$ and $R^{(0)}=0_{(n+d) \times (n+d)}$ respectively. At the end of the last iteration, we retrieve the orthogonal $Q=Q^{(T)}$ and the upper triangular $R=R^{(T)}$ as the output for $\widetilde{A} = QR$. 
We further consider the following submatrices of $Q^{(t)}$ and $ R^{(t)}$:
\begin{align*}
    &Q^{(t)} = \begin{bmatrix} Q_1^{(t)} \\ Q_2^{(t)} \end{bmatrix}, R^{(t)} = \begin{bmatrix} R_1^{(t)} & R_2^{(t)} \end{bmatrix}
\end{align*}
where $ Q_1^{(t)} $: $n \times (n+d)$,  $Q_2^{(t)} $: $c \times (n+d)$, $ R_1^{(t)} $: $(n+d) \times n$, and  $R_2^{(t)} $: $(n+d) \times d$. 
Lemma \ref{lem:2way_checksum} shows that the original vertical checksums $G_v A$ and horizontal checksums $A G_h$ are translated to checksums $G_v Q_1^{(t)}$ for $Q$-protection and $ R_1^{(t)} G_h$ for $R$-protection during the computation. 
% The proofs for Lemma \ref{lem:2way_checksum} and Corollary \ref{corol: final_form} can be found in ~\cite[Appendix \ref{appendixA:checksum_preserving}]{full_version}. 

\begin{lemma}[Lemma 1, \cite{qr_isit}]
\label{lem:2way_checksum}
For both sequential and parallel MGS, the following checksum relations hold for $t \in [0, T]$: 
\begin{align}
Q_2^{(t)}= G_v Q_1^{(t)} \label{eq:2way_checksum1}\\
R_2^{(t)}=  R_1^{(t)} G_h \label{eq:2way_checksum2}
\end{align}



\end{lemma}

\begin{comment}
\begin{proof}[Intuitive Proof:]
We present an intuitive proof for Equation (\ref{eq:2way_checksum}). From Algorithm \ref{alg: sequential_mgs}, we observe that each column $q_i$ of the $Q$-factor is on updated on line 6 by $q_i = u_i/r_{ii}$, so if the checksum relation holds for $u_i$, it also holds for $q_i$, i.e. for $q_i = \begin{bmatrix}q_{i1} \\ q_{i2}\end{bmatrix}$, we have $q_{i2} = G_v q_{i1}$. We can thus use induction on the iteration $t=0, \ldots, n+d$ to prove that the checksum relation holds for all $u_i$'s and $q_i$'s. The inductive step for $q_i$ is straight-forward. For $u_i$, it is only updated on line 9 by $u_j = u_j - r_{ij} q_i$. By the inductive hypothesis, we know that the checksum relation holds for $u_j$ in the previous  iteration and consequently $q_i$ in the current iteration, so we conclude the checksum relation holds for $u_j$ now. 
\end{proof}
\end{comment} 
\begin{corollary}[Corollary 1.1, \cite{qr_isit}]
\label{corol: final_form}
At the end of the QR decomposition, the factorization of $\widetilde{A}$ has the final form:
\begin{align}
\label{reduced_QR}
\widetilde{A} = \begin{bmatrix}
Q_1 \\
Q_2
\end{bmatrix} \begin{bmatrix}
R_1 &
R_2
\end{bmatrix}
=
\begin{bmatrix}
Q_1 \\
G_v Q_1
\end{bmatrix} \begin{bmatrix}
R_1 &
R_1 G_h
\end{bmatrix}
\end{align}
where $Q_i=Q_i^{(T)}$ and  $R_i=R_i^{(T)}$.
\end{corollary}


\begin{remark}
\textcolor{blue}{All the prevalent QR decomposition methods including Householder \cite{colchecksum, soft_error2}, Givens Rotations \cite{givens_rotations1} and MGS exhibit $R$-factor checksum-preservation. However, only MGS permits $Q$-factor checksum-preservation through  \eqref{eq:2way_checksum1} as above thanks to using linear projection of the input matrix's column vectors for orthogonalization. On the other hand, Householder and Givens Rotations respectively rely on the non-linear reflections and rotations, thereby undermining their $Q$-factor preservation, and thus .
 }

% Other prevalent QR decomposition methods including Householder \cite{colchecksum, soft_error2} and Givens Rotations \cite{givens_rotations1} do not possess $Q$-factor checksum-preservation, since their $Q$ matrix computation depends non-linearly on the column vectors of the input matrix $\widetilde{A}$. 

% While the R-factor checksum-preservation holds for Householder \cite{colchecksum, soft_error2}, Givens Rotations \cite{givens_rotations1} 

%     Remark after Lemma 1 explaining why checksum-preservation would not hold for other algorithms. 
\end{remark}


\textcolor{red}{[TODO] Explain why this doesn't apply to Householder or Givens.}
\subsection{Problem Formulation}

\textcolor{red}{[TODO] say that we deal with Q-factor and R-factor protection against \emph{multiple} failures.}

==> scrap.tex <==
% \begin{theorem}
% Let $\widetilde{G} = \begin{bmatrix} \widetilde{G}_1 & \widetilde{V} \end{bmatrix}$ be a $r$-by-$p_r$ matrix, where $\widetilde{V}$ is an $r$-by-$p_r$ matrix whose entries are chosen randomly from $\mathrm{Unif}(0,1)$ and $\widetilde{G}_1 = -\frac{1}{2} \widetilde{V} \widetilde{V}^T$ is an $r$-by-$r$ matrix. Then, for every square submatrix $S$ of $\widetilde{G}$ is full rank with probability 1. 
% \end{theorem}
% \begin{proof}
% Let $n_s$ denote the dimension of $S$. We can divide this into two cases: (i) When $S$ is a submatrix of $\widetilde{V}$, and (ii) when $t$ columns of $S$ are from $\widetilde{G}_1$ and $(n_s-t)$ columns are from $\widetilde{V}$ ($1 \leq n_s \leq r$, $0 \leq t \leq n_s$). It was already shown in the literature that every square submatrix of a random matrix is full rank with probability 1 (\hj{TODO: Find reference}). Thus, we will focus on the second case. 

% Let $\mathrm{Perm}(n_s)$ be all permutations of $\{1, \ldots, n_s\}$, and for permutation $\sigma$, $\sigma_i$ is the $i$-th element in the sequence. For example when $n_s = 3$, if $\sigma = [2 \;\; 3 \;\; 1]$, then $\sigma_1 =2, \sigma_2 = 3, \sigma_3=1$. The Leibniz formula for matrix determinant is:
% \begin{equation}
%     \mathrm{det}(S) = \sum_{\sigma \in \mathrm{Perm}(n_s)} \mathrm{sgn}(\sigma) \prod_{i=1}^{n_s} s_{i, \sigma_i} = \sum_{\sigma \in \mathrm{Perm}(n_s)} \xi(\sigma), \qquad \xi(\sigma) \triangleq \mathrm{sgn}(\sigma) \prod_{i=1}^{n_s} s_{i, \sigma_i}.
% \end{equation}
% $\mathrm{sgn}(\sigma)$ is $+1$ or $-1$, but since this term is not important for our argument, we refer to~\cite{linearalgebra} for more explanation \hj{TODO: Add reference}. 

% We now prove that $\mathrm{det}(S)$ is a non-zero polynomial in $v_{i,j}$'s.  Let us consider the term:
% \begin{equation}
%     \xi (\sigma = [ 1\;\; \ldots \;\; n_s]) = \prod_{i=1}^{n_s} s_{i, i}. 
% \end{equation}
% For simplicity, let us assume that the $t$ columns from $\widetilde{G}_1$ are $\mbg_1, \ldots \mbg_t$ and the $n_s -t$ columns of $\widetilde{V}$ are $\mbv_{1}, \ldots \mbv_{n_s-t}$. The argument naturally extends to a general case. Now, $\prod_{i=1}^{n_s} s_{i, i}$ can be expanded as:
% \begin{align}
%     \prod_{i=1}^{n_s} s_{i, i} &= \prod_{i=1}^{t} g_{i,i} \prod_{i=1}^{n_s -t} v_{i, t+i} \\ 
%     &= \left(-\frac{1}{2}\right)^t \cdot \left( \prod_{i=1}^t \sum_{j=1}^{p_r} v_{i,j}^2 \right) \cdot \prod_{i=1}^{n_s -t} v_{i, t+i}. \label{eq:det_expsn}
% \end{align}
% In \eqref{eq:det_expsn}, let us focus on one term: $(v_{1,p_r})^2 (v_{2, p_r-1})^2 \cdots (v_{t,p_r-t+1})^2 \cdot \prod_{i=1}^{n_s -t} v_{i, t+i} \triangleq \psi$. We show that this term does not appear anywhere else in $\xi (\sigma')$ when $\sigma' \neq [ 1\;\; \ldots \;\; n_s] $, and thus this term cannot be canceled out. We prove this by contradiction. 

% Assume there exists a $\sigma'$ such that $\psi \in \xi(\sigma')$. First, let us assume that there exists $1 \leq i \leq t$ such that $\sigma'_i = j \neq i$. We get the $v_{i, p_r-i+1}$ term only from $g_{i,j}$ and $g_{k,i}$ ($k \neq i$) as:
% \begin{align}
%     g_{i,j} &= v_{i,1}v_{j,1} + \cdots + v_{i,p_r-i+1}v_{j,p_r-i+1} + \cdots v_{i,p_r}v_{j,p_r} \\
%     g_{k,i} &= v_{k,1}v_{i,1} + \cdots + v_{k,p_r-i+1}v_{i,p_r-i+1} + \cdots v_{k,p_r}v_{i,p_r}.
% \end{align}
% Then, the only term that has $(v_{i, p_r-i+1})^2$ is the product of $v_{i,p_r-i+1}v_{j,p_r-i+1} $ and $v_{k,p_r-i+1}v_{i,p_r-i+1}$: 
% \begin{equation}
%     v_{i,p_r-i+1}^2 v_{j,p_r-i+1} v_{k,p_r-i+1}. 
% \end{equation}
% Notice that this term has $v_{j,p_r-i+1} v_{k,p_r-i+1}$ which was not present in $\psi$. Hence, $\psi \notin \xi(\sigma)$.

% Now, assume that there exists $t+1 \leq i \leq n_s$ such that $\sigma'_i = j \neq i$. Then, $\xi(\sigma')$ always has the term $v_{t+i, j}$ ($j \neq i$), which was not present in $\psi$. Hence, $\psi \notin \xi(\sigma)$. 

% This proves that $\psi$ appears only in $\xi(\sigma = [1 \;\; \cdots \;\; n_s])$ and hence this term has a a non-zero coefficient, $(-1/2)^t$. As $\mathrm{Pr}(\{v_{i,j}\}_{\substack{i=1,\ldots,r, \\ j=1, \ldots, p_r}}: p(\{ v_{i,j}\}) =0) = 0$ for a non-zero polynomial $p$, this completes the proof.
% \end{proof}

\subsection{Proof of In-node Checksum Lower Bound}
% \begin{definition}[Load-balanced In-node Checksum Distribution]\label{def:innode_distr}
% Let $P$ be the total number of nodes and let $K$ be the number of checksum blocks. Then, we say the checksum distribution is load-balanced if:
% \begin{itemize}
%     \item $\overline{a} \triangleq K - P\floor{\frac{K}{P}}$ of the nodes have $\ceil{\frac{K}{P}}$ checksum blocks, and
%     \item $\overline{b} \triangleq P - K + P\floor{\frac{K}{P}}$ of the nodes have $\floor{\frac{K}{P}}$ checksum blocks.
% \end{itemize}
% \end{definition}

% \begin{lemma}\label{lem:in_node_lb}
% Under the load-balanced in-node checksum distribution, to recover from any $r$ failed nodes out of $P$ nodes, the number of checksums $K$ must satisfy:
% \begin{equation} \label{eq:in_node_lem}
%   a \ceil{\frac{K}{P}} + b \floor{\frac{K}{P}} \geq \; r \frac{L}{P}
% \end{equation}
% for any $a+b = P-r$ and $a \leq \overline{a}$ and $b \leq  \overline{b}$.
% \end{lemma}
% \begin{proof}
% Assume there exists $a'$ and $b'$ such that $a'+b' = P-r$, $a' \leq \overline{a}$, $b' \leq \overline{b}$ that satisfy: 
% \begin{equation} 
%   a' \ceil{\frac{K}{P}} + b' \floor{\frac{K}{P}} < r \frac{L}{P}.
% \end{equation}
% When $a'$ nodes with $\ceil{\frac{K}{P}}$ 

% \end{proof}

% \begin{construction}[In-Node Systematic MDS Coding] \label{const:in_node}
% Let $D_1, \ldots, D_L$ be data blocks and $C_1, \ldots C_K$ be checksum blocks, and let $P$ be the number of nodes. We assume that $P$ divides $L$ and we assume the load-balanced setting, i.e, each node has $L/P$ data blocks and the checksum distribution follows the load-balanced in-node checksum distribution. Let $\mathcal{I}_p$ be the set of data block indices in the $p$-th node and let $\mathsf{Proc}(D_i)$  or $\mathsf{Proc}(C_i)$  denote the processor index the data or checksum block belongs to. 
% Let $\tilG \in \bbR^{K \times \frac{(P-1)L}{P}}$ be a checksum-generating matrix of a $(K+(P-1)\frac{L}{P}, (P-1)\frac{L}{P})$ systematic MDS code. Then, In-Node Systematic MDS Coding encodes the $i$-th checksum block $C_i$ as follows:
% \begin{equation} \label{eq:in_node_cksum}
%     C_i = \sum_{j \notin \mathcal{I}_{\mathsf{Proc}(C_i)}} \tilG_{i,j} D_j
% \end{equation}
% \end{construction}

% \begin{lemma} \label{lem:in_node_mds}
% In-node systematic MDS coding given in Construction~\ref{const:in_node} with $K$ that satisfies \eqref{eq:in_node_lem} can tolerate any $r$ failed nodes out of $P$ nodes. 
% \end{lemma}
% \begin{proof}
% From any $P-r$ survived nodes, we have $(P-r)\frac{L}{P}$ data blocks and $r\frac{L}{P}$ checksum blocks as $K$ satisfies the condition in \eqref{eq:in_node_lem}. Let $p_1, \ldots, p_r$ be the index of failed nodes. After subtracting the data blocks from the survived nodes, the checksum equations given in \eqref{eq:in_node_cksum} reduces to equations in $r\frac{L}{P}$ data blocks as follows: 
% \begin{equation}
%      C_i = \sum_{j \in \cup_{k=1}^{r} \mathcal{I}_{p_{k}}} \tilG_{i,j} D_j.
% \end{equation}
% We have $r\frac{L}{P}$ such equations and since any square submatrix of $\tilG$ is full-rank, we can solve the set of linear equations to retrieve $D_j$'s for $j \in \cup_{k=1}^{r} \mathcal{I}_{p_{k}}$.
% \end{proof}

% \begin{theorem} \label{thm:in_node_opt}
% Let $L$ be the number of data blocks and assume that the total number of nodes $P$ divides $L$. Under the load-balanced in-node checksum distribution, to recover from any $r$ failed nodes out of $P$ nodes, 
% \begin{equation}
% K = \frac{rL}{P} + r \ceil{\frac{rL}{(P-r)P}}    
%  \end{equation}
% is the optimum number of checksum blocks required. 
% \end{theorem}
% \begin{proof}
% % First, information-theoretically, the number of checksum blocks remaining must be at least the number of systematic blocks lost from the $r$ failed nodes: 
% % \begin{equation} \label{eq:inf_thr_lb}
% %   a \ceil{\frac{K}{P}} + b \floor{\frac{K}{P}} \geq \; r \frac{L}{P}
% % \end{equation}
% % for any $a+b = P-r$ and $a \leq K - P\floor{\frac{K}{P}} \triangleq \overline{a}$ and $b \leq P - K + P\floor{\frac{K}{P}} \triangleq \overline{b}$. Note that $\overline{a}$ and $\overline{b}$ are the total number of nodes with $\ceil{\frac{K}{P}}$ checksum blocks and $\floor{\frac{K}{P}}$ checksum blocks, respectively, as defined in Definition~\ref{def:innode_distr}. 
% By Lemma 1, we have: 
% \begin{equation} \label{eq:inf_thr_lb}
%   a \ceil{\frac{K}{P}} + b \floor{\frac{K}{P}} \geq \; r \frac{L}{P}
% \end{equation}
% for any $a+b = P-r$ and $a \leq \overline{a}$ and $b \leq  \overline{b}$.
% As this has to be satisfied for the worst case $a$ and $b$, let us consider:
% \begin{equation}
%     \min_{\substack{a,b \geq 0, \; a+b =r, \\ a \leq \overline{a}, \; b \leq \overline{b}}}  a \ceil{\frac{K}{P}} + b \floor{\frac{K}{P}} = \begin{cases} (P-r) \floor{\frac{K}{P}} & \text{ if } \overline{b} \geq P- r\\ 
%     (P-r-\overline{b}) \ceil{\frac{K}{P}} + \overline{b} \floor{\frac{K}{P}}  & \text{ otherwise. }\end{cases}
% \end{equation}
% Note that for any $K$, $(P-r) \ceil{\frac{K}{P}}  \geq (P-r) \floor{\frac{K}{P}}$ and  $(P-r) \ceil{\frac{K}{P}}  \geq (P-r-\overline{b}) \ceil{\frac{K}{P}} + \overline{b} \floor{\frac{K}{P}} $. Hence, 
% \begin{equation}
%     (P-r) \ceil{\frac{K}{P}} \geq \min_{\substack{a,b \geq 0, \; a+b =r, \\ a \leq \overline{a}, \; b \leq \overline{b}}}  a \ceil{\frac{K}{P}} + b \floor{\frac{K}{P}}  \geq r \frac{L}{P}.
% \end{equation}
% Because $\ceil{\frac{K}{P}} $ is an integer,
% \begin{equation}
%     \ceil{\frac{K}{P}} \geq \ceil{\frac{rL}{(P-r)P}}.
% \end{equation}
% Now, let us find $K$ such that $\ceil{\frac{K}{P}}  = \ceil{\frac{rL}{(P-r)P}}$ that satisfy \eqref{eq:inf_thr_lb}. Then, $K$ be expressed as $K = P \ceil{\frac{rL}{(P-r)P}} - m$ where $m = 0, \ldots, P-1$. We will try to find the largest $m$, and we divide these into three cases: i) $m \geq P-r$, ii) $0 < m < P-r$, and iii) $m = 0$. 

% Case i) $m \geq P-r$: Notice that $\overline{b} = m \geq P- r$, and thus we have:
% \begin{align}
%     \min_{\substack{a,b \geq 0, \; a+b =r, \\ a \leq \overline{a}, \; b \leq \overline{b}}}  a \ceil{\frac{K}{P}} + b \floor{\frac{K}{P}} &=  (P-r) \floor{\frac{K}{P}} \nonumber \\
%     &=  (P-r) \left( \ceil{\frac{rL}{(P-r)P}}-1 \right). \label{eq:thm_lb_prf1} 
% \end{align}
% When $\frac{rL}{(P-r)P}$ is an integer, 
% \begin{align*}
%     \eqref{eq:thm_lb_prf1} = (P-r)\left(\frac{rL}{(P-r)P}-1 \right) < \frac{rL}{P}.
% \end{align*}
% When $\frac{rL}{(P-r)P}$ is not an integer, 
% \begin{align*}
%     \eqref{eq:thm_lb_prf1} = (P-r)\floor{\frac{rL}{(P-r)P}} < \frac{rL}{P}.
% \end{align*}
% Hence, there does not exist $m \geq P-r$ that satisfies \eqref{eq:inf_thr_lb}.

% Case ii) $0 < m < P-r$: As  $\overline{b} = m < P- r$, we have:
% \begin{align*}
%     \min_{\substack{a,b \geq 0, \; a+b =r, \\ a \leq \overline{a}, \; b \leq \overline{b}}}  a \ceil{\frac{K}{P}} + b \floor{\frac{K}{P}} &=  (P-r-\overline{b}) \ceil{\frac{K}{P}} + \overline{b} \floor{\frac{K}{P}} \\
%     &=  K - r \left( \floor{\frac{K}{P}}+1 \right ) = K -r\ceil{\frac{K}{P}} \\ 
%     &= K - r\ceil{\frac{rL}{(P-r)P}} \geq \frac{rL}{P}
% \end{align*}
% Hence, $K = r\ceil{\frac{rL}{(P-r)P}} +\frac{rL}{P}$ satisfy \eqref{eq:inf_thr_lb}. We can also check that: 
% \begin{align*}
%  m &= P\ceil{\frac{rL}{(P-r)P}} - K   \\ 
%  &=P\ceil{\frac{rL}{(P-r)P}} - r\ceil{\frac{rL}{(P-r)P}} - \frac{rL}{P} \\ 
%  &= (P-r)\ceil{\frac{rL}{(P-r)P}}-\frac{rL}{P} < P-r.
% \end{align*}

% As we already found $m$ in Case ii), we do not have to consider Case iii). 

% Finally, by Lemma~\ref{lem:in_node_mds}, the coding scheme given in Construction~\ref{const:in_node} with $K = r\ceil{\frac{rL}{(P-r)P}} +\frac{rL}{P}$ can tolerate any $r$ failures out of $P$ nodes.
% \end{proof}



% \begin{theorem}
% Let $L$ be the number of data blocks and assume that the total number of nodes $P$ divides $L$. To recover from any $r$ failed nodes out of $P$ nodes, under the load-balanced in-node checksum distribution, the number of checksum blocks required is bounded by:
% \begin{equation}
%     K \geq \frac{rL}{P-r}. 
% \end{equation}
% \end{theorem}


% \begin{proof}
% First, information-theoretically, the number of checksum blocks remaining must be at least the number of systematic blocks lost from the $r$ failed nodes: 
% \begin{equation} \label{eq:inf_thr_lb}
%     K - \left( a \ceil{\frac{K}{P}} + b \floor{\frac{K}{P}} \right) \geq \; r \frac{L}{P}
% \end{equation}
% for any $a, b \geq 0$ such that $a+b = r$ and $a \leq K - P\floor{\frac{K}{P}} \triangleq \overline{a}$ and $b \leq P - K + \floor{\frac{K}{P}} \triangleq \overline{b}$. Note that $\overline{a}$ and $\overline{b}$ are the total number of nodes with $\ceil{\frac{K}{P}}$ checksum blocks and $\floor{\frac{K}{P}}$ checksum blocks, respectively, as defined in Definition~\ref{def:innode_distr}. 

% When we have $\ceil{\frac{K}{P}} = \floor{\frac{K}{P}} = \frac{K}{P}$, \eqref{eq:inf_thr_lb} is simply: 
% \begin{equation} \label{eq:lb_prf2}
%     K - r \frac{K}{P} \geq r \frac{L}{P} \iff K \geq \frac{rL}{P-r}. 
% \end{equation}

% Let us now focus on when $\ceil{\frac{K}{P}} \neq \floor{\frac{K}{P}}$, i.e., $\ceil{\frac{K}{P}} = \floor{\frac{K}{P}} +1$.  First, assume $r < \overline{a} $. Then,
% \begin{align*}
%     \min_{\substack{a,b \geq 0, \; a+b =r, \\ a \leq \overline{a}, \; b \leq \overline{b}}}  K - \left( a \ceil{\frac{K}{P}} + b \floor{\frac{K}{P}} \right)  = K - r \ceil{\frac{K}{P}} \geq \; r \frac{L}{P}
% \end{align*} 

% Since $K - r \frac{K}{P}  \geq K - r \ceil{\frac{K}{P}} $, this again reduces to \eqref{eq:lb_prf2}.
% % \begin{equation*}
% %     K - r \frac{K}{P} \geq r \frac{L}{P} \iff K \geq \frac{rL}{P-r}. 
% % \end{equation*}

% Now, let us consider when $ r \geq  \overline{a} $. Then, 
% \begin{align*}
%     \min_{\substack{a,b \geq 0, \; a+b =r, \\ a \leq \overline{a}, \; b \leq \overline{b}}} K - \left( a \ceil{\frac{K}{P}} + b \floor{\frac{K}{P}} \right) &= K - \overline{a} \ceil{\frac{K}{P}} - (r-\overline{a}) \floor{\frac{K}{P}} \\
%     &= K -  \left(K - P\floor{\frac{K}{P}} \right) \ceil{\frac{K}{P}} - \left(r -  K + P\floor{\frac{K}{P}} \right) \floor{\frac{K}{P}} \\ 
%     &= 
%     K -  \left(K - P\floor{\frac{K}{P}} \right) \left( \floor{\frac{K}{P}} + 1 
%     \right)
%     - \left(r -  K + P\floor{\frac{K}{P}} \right) \floor{\frac{K}{P}}
%      \\ 
%     &= (P-r) \floor{\frac{K}{P}} \geq r \frac{L}{P}.
% \end{align*} 
% Hence, 
% \begin{align*}
%     (P-r) \frac{K}{P} \geq (P-r) \floor{\frac{K}{P}} \geq r \frac{L}{P} \iff K \geq \frac{rL}{P-r}.
% \end{align*}


% \end{proof}

\clearpage


\section{MDS properties}
Let $G$ be a checksum generating matrix for row-wise checksums, which has dimension $c \times n$ where $c$ is a multiple of $n/p_r$. Assuming that we use the same encoding coefficients at each node, $G$ can be represented as: 
\begin{equation}
    G = \widetilde{G} \otimes I_{n/p_r},
\end{equation}
where $\otimes$ is a Kronecker product, $\widetilde{G}$ is an $r \times p_r$ matrix, and $r$ is the number of checksum nodes per column. 

For example, for $r=2$, $G$ can be written as: \begin{equation}
    G = \begin{bmatrix} 
    \widetilde{G}_{1,1} I_{n/p_r} & \ldots & \widetilde{G}_{1,p_r} I_{n/p_r} \\ 
    \widetilde{G}_{2,1} I_{n/p_r} & \ldots & \widetilde{G}_{2,p_r} I_{n/p_r}
    \end{bmatrix}.
\end{equation}



We know how to design a good matrix $\tilde{G}$. The desirable MDS property translates into the property of the matrix $\tilde{G}$:
\begin{theorem}
$\tilde{G}$ has the MDS property if and only if every square submatrix of $\tilde{G}$ is full-rank. 
\end{theorem}
\begin{lemma}[Equivalence of post-orthogonalization condition]
The following holds:
\begin{align}
    G_1 = -\frac{1}{2} V V^T \iff \widetilde{G_1} = -\frac{1}{2} \widetilde{V} \widetilde{V}^T
\end{align} 



\end{lemma}
\begin{proof}
We have:
\begin{align*}
     G_1 = -\frac{1}{2} V V^T  &\iff  \widetilde{G_1} \otimes I_{n/p_r} = -\frac{1}{2} (\widetilde{V} \otimes I_{n/p_r}) (\widetilde{V}^T \otimes I_{n/p_r}) \\
     & \iff  \widetilde{G_1} \otimes I_{n/p_r}  = (-\frac{1}{2} \widetilde{V} \widetilde{V}^T) \otimes I_{n/p_r} 
\end{align*}
\end{proof}
